Beyond Sharing Weights for Deep Domain Adaptation

The performance of a classifier trained on data coming from a specific domain typically degrades when applied to a related but different one. While annotating many samples from the new domain would address this issue, it is often too expensive or impractical. Domain Adaptation has therefore emerged as a solution to this problem; It leverages annotated data from a source domain, in which it is abundant, to train a classifier to operate in a target domain, in which it is either sparse or even lacking altogether. In this context, the recent trend consists of learning deep architectures whose weights are shared for both domains, which essentially amounts to learning domain invariant features. Here, we show that it is more effective to explicitly model the shift from one domain to the other. To this end, we introduce a two-stream architecture, where one operates in the source domain and the other in the target domain. In contrast to other approaches, the weights in corresponding layers are related but not shared. We demonstrate that this both yields higher accuracy than state-of-the-art methods on several object recognition and detection tasks and consistently outperforms networks with shared weights in both supervised and unsupervised settings.

==> fig/office.tex <==
\begin{table}[!h]
	\centering
	\begin{tabularx}{\linewidth}{XM{1.2cm}M{1.2cm}M{1.2cm}M{1.2cm}}
		\toprule
		& \multicolumn{4}{c}{Accuracy} \\
		\cmidrule{2-5}
		
		& A $\rightarrow$ W & D $\rightarrow$ W & W $\rightarrow$ D  & Average\\
		GFK~\cite{Gong12b}		  	& 0.464 & 0.613 & 0.663 & 0.530 \\
		SA~\cite{Fernando13}			& 0.450 & 0.648 & 0.699 & 0.599 \\
		DA-NBNN~\cite{Tommasi13}		& 0.528 & 0.766 & 0.762 & 0.685 \\
		DLID~\cite{Chopra13} 			& 0.519 & 0.782 & 0.899 & 0.733 \\
		DeCAF$_6$+T~\cite{Donahue13a} 		& 0.807 & 0.948 & - 	& - \\
		DaNN~\cite{Ghifary14}			& 0.536 & 0.712 & 0.835 & 0.694 \\
		DDC~\cite{Tzeng14}			& 0.841 & {\bf 0.954} & 0.963 & 0.919 \\
		Ours					& {\bf 0.876} & 0.949 & {\bf 0.988} & {\bf 0.938} \\
		\bottomrule
	\end{tabularx}
	\caption{Comparison to other domain adaptation techniques on the Office standard benchmark. We evaluate on all 31 categories, according to the standard evaluation protocol, described in~\cite{Saenko10}.}
	\label{tbl:Domain_adapt_OF}
\end{table}

